A block inertial Bregman proximal algorithm for nonsmooth nonconvex problems with application to symmetric nonnegative matrix tri-factorization

We propose BIBPA, a block inertial Bregman proximal algorithm for minimizing the sum of a block relatively smooth function (that is, relatively smooth concerning each block) and block separable nonsmooth nonconvex functions. We prove that the sequence generated by BIBPA subsequentially converges to critical points of the objective under standard assumptions, and globally converges when the objective function is additionally assumed to satisfy the Kurdyka-{\L}ojasiewicz (K{\L}) property. We also provide the convergence rate when the objective satisfies the {\L}ojasiewicz inequality. We apply BIBPA to the symmetric nonnegative matrix tri-factorization (SymTriNMF) problem, where we propose kernel functions for SymTriNMF and provide closed-form solutions for subproblems of BIBPA.

==> Preamble.tex <==
%	\usepackage[%
%		eqreset=section,
%		thmreset=section,
%	% 	noload={caption,subcaption},
%	 ]{myPreamble}
\usepackage{todonotes}
%\usepackage{bm}

\CreateNewTheorem[Fact]{fact}[dummythm]{Fact}

% change operator font (default is bold)
% \makeatletter
%    \renewcommand\operator@font{\rm}
% \makeatother

% Notation for big vectors. Uncomment/change the command \bm to whatever you want
% \renewcommand\bm[1]{#1} % Removes bold face
% Usage: \bm{x}^k or simply \bm x^k

\newcommandx\p[3][1=\gamma,3=h]{\prox_{#1#2}^{#3}}

\newcommand\C{\mathcal C}
\makeatletter
	\newcommand\D[1][h_i]{%
		\@ifnextchar_{\operatorname D}{%
			\ifstrempty{#1}{\operatorname D}{\operatorname D_{#1}}%
		}
	}
	%
\makeatother
\newcommandx\FBE[2][1={f,g},2={\gamma h_i}]{\varphi_{#2}^{#1}}
\newcommandx\T[2][2={\nicefrac{h_i}{\gamma_i^k}},1={ }]{\operatorname T_{#2}^{#1}}
\newcommandx\M[2][2={\nicefrac{h_i}{\gamma_i^k}},1={ }]{\operatorname{\mathcal{M}}_{#2}^{#1}}
\newcommandx\TG[2][1={f,g},2={\gamma^k h_i}]{\operatorname T_{#2}^{#1}}
\newcommandx\RGH[2][1={f,g},2={\gamma h_i}]{\operatorname R_{#2}^{#1}}
\let\proj\relax
\DeclareMathOperator\proj{Proj}

%% Custom creferencing of BIBPA
	\newcommand\refBIBPA[1][ (\cref{alg:bibpa})]{%
		\hyperref[alg:bibpa]{{\tt\textsc{BIBPA}}}#1%
	}%

